Contrastive Hierarchical Discourse Graph for Scientific Document Summarization

The extended structural context has made scientific paper summarization a challenging task. This paper proposes CHANGES, a contrastive hierarchical graph neural network for extractive scientific paper summarization. CHANGES represents a scientific paper with a hierarchical discourse graph and learns effective sentence representations with dedicated designed hierarchical graph information aggregation. We also propose a graph contrastive learning module to learn global theme-aware sentence representations. Extensive experiments on the PubMed and arXiv benchmark datasets prove the effectiveness of CHANGES and the importance of capturing hierarchical structure information in modeling scientific papers.

==> content/motivation.tex <==
\section{Motivation}
\subsection{Scientific summarization benchmarks}
Existing large-scale summarization datasets are mainly relatively short documents, such as CNN/DailyMail \cite{hermann2015teaching}, XSum \cite{narayan2018ranking} and New York Times \cite{sandhaus2008new} for news summarization, SAMSum \cite{gliwa2019samsum} for dialogue summarization. Recently, \citet{cohan2018discourse} introduced two large-scale datasets of long and structured scientific papers obtained from ArXiv
and PubMed repositories. The abstract section of papers are used as the reference summaries (ground truth). For extractive summarization task, we follow the convention in \cite{narayan2018ranking} and greedily extract ground truth sentences to maximize the ROUGE-1 score of the reference summary.

\input{table/stat}
Detailed statistics of ArXiv
and PubMed datasets are shown in Table . These two scientific paper datasets contain
much longer documents and richer discourse structure information, and are widely used as benchmarks for long document summarization. Thus, we use these two datasets to explore the pattern of long document summarization.

\subsection{Benchmark Analysis} 
\paragraph{Section Bias}
Scientific documents contain clear section structures, so we devide the sections into five categories: pre-intro, introduction, body, conclusion, and post conclusion. The ground truth sentences distribution with respect to the section is shown in Figure. We notice lead bias still exists in long documents since pre-intro sections tend to contain much more salient sentences compared to the rest of the sections. Surprisingly, we find the body sections barely contain salient information in spite of it is the category with longest length. We argue this is due to the writing convention that body section tend to contain too many technical details, which makes the sentences less salient with respect to the whole document.




\paragraph{Position Bias}
We show how extractive ground truth summaries distribute inter and intra different sections in Figure  and Figure . We could notice that sentences within the same section seems to have a more obvious positional bias. It agrees with normal writing convention that
first few sentences and last few sentences tend to be summative and informative.

Based on all these patterns, we propose a heterogeneous graph neural network for scientific paper summarization.

\begin{figure}
\centering
\subfigure{
\includegraphics[width=0.45\textwidth]{figure/ArXiv_rouge_dist.png}}
\subfigure{
\includegraphics[width=0.45\textwidth]{figure/PubMed_rouge_dist.png}}
\caption{ROUGE score distribution of PubMed and ArXiv datasets}
\label{rouge_dis}
\end{figure}

\begin{figure}
\centering
\subfigure{
\includegraphics[width=0.2\textwidth]{figure/ArXiv gt dist.png}}
\subfigure{
\includegraphics[width=0.2\textwidth]{figure/PubMed gt dist.png}}
\caption{Oracle GT distribution for each section}
\label{section_dis}
\end{figure}





\begin{figure}
\centering
\subfigure{
\includegraphics[width=0.2\textwidth]{figure/ArXiv gt sec dist.png}}
\subfigure{
\includegraphics[width=0.2\textwidth]{figure/PubMed gt sec dist.png}}
\caption{Oracle GT distribution for each section}
\label{oracle_dis}
\end{figure}


==> table/arxiv_ablation.tex <==
\begin{table}[htbp]
\centering
\small
\begin{tabular}{c| c c c}
    \hline Model & ROUGE-1 & ROUGE-2 & ROUGE-L \\
    \hline \textbf{\model} & \textbf{45.61} & \textbf{18.02} & \textbf{40.06} \\
     w/o ContraMask & 45.34 & 17.22 & 39.83 \\
     w/o ContraFeature & 44.47  & 16.58 & 38.87 \\

     w/o Contra & 44.35 & 16.44 & 38.52 \\
     w/o HeterGraph & 44.72 & 16.79 & 39.10 \\
    \hline
\end{tabular}
\label{ablation_arxiv}
\caption{Ablation Results of removing components of our model on ArXiv Dataset}
\end{table}

==> table/arxiv_result.tex <==
\begin{table}[htbp]
\centering
\small
\resizebox{0.5\textwidth}{!}{

\begin{tabular}{|c | c | c | c|}
    \hline 
    \textbf{Model} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} \Tstrut\Bstrut\\
    \hline SumBasic & 29.47 & 6.95 & 26.30 \\
    LSA & 29.91 & 7.42 & 25.67 \\
    LexRank & 33.85  & 10.73 & 28.99 \\
    
    \hline Lead & 33.66 & 8.94 & 22.19 \\
    PACSUM & 38.57 & 10.93 & 34.33 \\
    HIPORANK & 39.34 & 12.56 & 34.89 \\
    Oracle & 53.88 & 23.05 & 34.90 \\

    \hline SentCLF & 34.01 & 8.71 & 30.41\\
    SentPTR & 42.32 & 15.63 & 38.06 \\
    Cheng\&Lapata & 42.24 & 15.97 & 27.88 \\
    SummaRuNNer & 42.81 & 16.52 & 28.23 \\
    ExtSum-LG & 43.62 & 17.36 & 29.14 \\
    ExtSum-LG + RdLoss & 44.01 & 17.79 & 39.09\\
    ExtSum-LG + MMR-Select+ & 43.87 & 17.50 & 38.97\\
    
    
    \hline PGN & 32.06 & 9.04 & 25.16 \\
    DiscourseAware & 35.80 & 11.05 & 31.80\\
    TLM-I+E & 41.62 & 14.69 & 38.03 \\
    
    \hline Ours & \textbf{45.56} & \textbf{17.74} & 29.36 \\
    \hline
\end{tabular}}
\caption{Results on PubMed Dataset}
\end{table}
